Scalable and Order-robust Continual Learning with Additive Parameter Decomposition

While recent continual learning methods largely alleviate the catastrophic problem on toy-sized datasets, some issues remain to be tackled to apply them to real-world problem domains. First, a continual learning model should effectively handle catastrophic forgetting and be efficient to train even with a large number of tasks. Secondly, it needs to tackle the problem of order-sensitivity, where the performance of the tasks largely varies based on the order of the task arrival sequence, as it may cause serious problems where fairness plays a critical role (e.g. medical diagnosis). To tackle these practical challenges, we propose a novel continual learning method that is scalable as well as order-robust, which instead of learning a completely shared set of weights, represents the parameters for each task as a sum of task-shared and sparse task-adaptive parameters. With our Additive Parameter Decomposition (APD), the task-adaptive parameters for earlier tasks remain mostly unaffected, where we update them only to reflect the changes made to the task-shared parameters. This decomposition of parameters effectively prevents catastrophic forgetting and order-sensitivity, while being computation- and memory-efficient. Further, we can achieve even better scalability with APD using hierarchical knowledge consolidation, which clusters the task-adaptive parameters to obtain hierarchically shared parameters. We validate our network with APD, APD-Net, on multiple benchmark datasets against state-of-the-art continual learning methods, which it largely outperforms in accuracy, scalability, and order-robustness.

==> cifar_table.tex <==
\begin{table*}
\tiny
\begin{center}
%\caption{Comparison of model.}
\caption{\small Experimenta results on CIFAR 100-split and CIFAR 100-superclass datasets. The results are the mean accuracies over $3$ run of experiments with random splits, performed with $5$ different task order sequences. STL is the single-task learing model that trains a separate network for each task independently.}
\small
\begin{tabular}{c|| c|c|c|c || c|c|c|c}
\hline 
\multicolumn{1}{c||}{}&\multicolumn{4}{c||}{CIFAR100-Split}&\multicolumn{4}{c}{CIFAR100-Superclass} \\
\hline \hline
  Methods & Capacity & Accuracy & AOPD & MOPD & Capacity & Accuracy & AOPD & MOPD  \\
\hline
STL			&
1,000\% & 63.75\% & 0.98\% & 2.23\% & 
2,000\% & 61.00\% & 2.31\% & 3.33\%  \\
\hdashline
L2T &
100\% 	& 48.73\% &  8.62\% 	& 17.77\% & 
100\% 	& 41.40\% &  8.59\% 	& 20.08\%\\
EWC ~\cite{kirkpatrick2017overcoming} &
100\% 	& 53.72\% & 7.06\% 	& 15.37\% & 
100\% 	& 47.78\% & 9.83\% 	& 16.87\%\\
P\&C~\citep{schwarz2018progress} &
100\% & 53.54\% & 6.59\% & 11.80\% & 
100\% & 48.42\%  & 9.05\% & 20.93\%\\
\hdashline
PGN ~\cite{RusuA2016nips}&
%174\% & 57.52\% & 7.29\% & 11.03\% & 
174\% & 55.71\% & 6.48\% & 11.10\% & 
300\% & 48.15\%  & 12.95\% & 19.27\%\\
DEN~\citep{YoonJ2018iclr}&
%174\% & 57.89\% & 6.11\% &10.92\% &
%186\% & 56.35\% & 9.13\% &13.97\% &
181\% & 57.38\% & 8.33\% &13.67\% &
191\% & 51.10\% & 5.35\% & 10.33\% \\
RCL~\citep{xu2018reinforced} &
181\% & 55.26\% &  5.90\% & 11.50\% & 
%189\% & 51.02\%  & 5.64\% & 16.00\% \\
184\% & 51.99\%  & 4.98\% & 14.13\% \\
\hline
HDN-Fixed&
%140\% & 59.43\% & 2,21\% & 3.30\% &  %logs/190525_cifar100_moracle_fixed_4p5e4
%139\% & 59.31\% & 2,42\% & 4.53\% &  %logs/190525_cifar100_moracle_fixed_4p5e4_app10
132\% & 59.32\% & 2.43\% & 4.03\% &  %logs/190525_cifar100_moracle_fixed_as_5e4
% 137\% & 56.04\% & 2.95\% & \bf{5.53}\% \\
128\% & 55.75\% & 3.16\% & 6.80\% \\ %logs/190525_cifar100_sup_moracle_fixed_as_6e4
%& 174\% & \bf{60.69}\% & \bf{1.46}\% & \bf{2.13}\% &
%& 171\% & \bf{60.39}\% & \bf{1.87}\% & \bf{2.67}\% & %logs/190525_cifar100_moracle_fixed_3e4_app10
& 175\% & \bf{61.02}\% & 2.26\% & \bf{2.87}\% & %logs/190525_cifar100_moracle_fixed_as_2p9e4
%& 161\% & 60.33\% & 2,33\% & 3.73\% &
% 181\% & \bf{57.36}\% & \bf{2.59}\% & \bf{5.20}\% \\ %logs/190525_cifar100_sup_moracle_fixed_3e4_app10
%  182\% & \bf{57.42}\% & \bf{2.68}\% & \bf{4.60}\% \\
191\% & \bf{57.98}\% & \bf{2.58}\% & \bf{4.53}\% \\ %logs/190525_cifar100_sup_moracle_fixed_as_3e4
HDN($1$)&
134\% & 59.93\% & 2.12\% & 3.43\% & %logs/190513_cifar100_moracle_l1_5e4_full_tau
133\% & 56.76\% & 3.02\% & 6.20\% \\ %logs/190515_cifar100_sup_moracle_6e4
& 170\% & \bf{61.30}\% & \bf{1.57}\% & \bf{2.77}\% & %logs/190422_cifar100_moracle_2p9e4_full_tau
191\% & \bf{58.37}\% & \bf{2.64}\% & \bf{5.47}\% \\ %190515_cifar100_sup_moracle_3e4
HDN($2$)&
135\% & \bf{60.74}\% & \bf{1.79}\% & 3.43\% &  %logs/190511_cifar100_moracle_reordered_base_l14e4_local_shared
130\% & 56.81\%  & \bf{2.85}\% & \bf{5.73}\% \\ %logs/190515_cifar100_sup_moracle_6e4_local_sharing
&
153\% & \bf{61.18}\% & \bf{1.86}\% & \bf{3.13}\% &  %logs/190511_cifar100_moracle_reordered_base_local_shared
182\% & \bf{58.53}\% & \bf{2.75}\% & \bf{5.67}\% \\  %logs/190516_cifar100_sup_moracle_3e4_k3n10_local_sharing
%193\% & \bf{58.44}\%  & \bf{2.62}\% & \bf{5.80}\% \\
\end{tabular}
\label{tab:main_table}
\vspace{-0.2in}
\end{center}
\end{table*}

% CIFAR100-SUPER
% ORACLE: l1=3e-4 / 6e-4
% ORACLE-LS: l1=3e-4 / 5e-4   ,k=3 per 10


==> cifar_table_hdn.tex <==
\clearpage
\begin{table*}
\tiny
\begin{center}
%\caption{Comparison of model.}
\caption{\small Full experiment results on CIFAR-100 Split and CIFAR-100 Superclass datasets. The results are the mean accuracies over $3$ runs of experiments with random splits, preformed with $5$ different task order sequences..}
\small
\begin{tabular}{c|| c|c|c|c || c|c|c|c}
\hline 
\multicolumn{1}{c||}{}&\multicolumn{4}{c||}{CIFAR-100 Split}&\multicolumn{4}{c}{CIFAR-100 Superclass} \\
\hline \hline
  Methods & Capacity & Accuracy & AOPD & MOPD & Capacity & Accuracy & AOPD & MOPD  \\
\hline
STL			&
1,000\% & 63.75\% & 0.98\% & 2.23\% & 
2,000\% & 61.00\% & 2.31\% & 3.33\%  \\
\hdashline
L2T &
100\% 	& 48.73\% &  8.62\% 	& 17.77\% & 
100\% 	& 41.40\% &  8.59\% 	& 20.08\%\\
EWC &
100\% 	& 53.72\% & 7.06\% 	& 15.37\% & 
100\% 	& 47.78\% & 9.83\% 	& 16.87\%\\
P\&C &
100\% & 53.54\% & 6.59\% & 11.80\% & 
100\% & 48.42\%  & 9.05\% & 20.93\%\\
\hdashline
PGN&
%174\% & 57.52\% & 7.29\% & 11.03\% & 
171\% & 54.90\% & 8.08\% & 14.63\% & 
271\% & 50.76\%  & 8.69\% & 16.80\%\\
DEN&
%174\% & 57.89\% & 6.11\% &10.92\% &
%186\% & 56.35\% & 9.13\% &13.97\% &
181\% & 57.38\% & 8.33\% &13.67\% &
191\% & 51.10\% & 5.35\% & 10.33\% \\
RCL&
181\% & 55.26\% &  5.90\% & 11.50\% & 
%189\% & 51.02\%  & 5.64\% & 16.00\% \\
184\% & 51.99\%  & 4.98\% & 14.13\% \\
\hline
APD-Fixed&
132\% & 59.32\% & 2.43\% & 4.03\% &  %logs/190525_cifar100_moracle_fixed_as_5e4
128\% & 55.75\% & 3.16\% & 6.80\% \\ %logs/190525_cifar100_sup_moracle_fixed_as_6e4
& 175\% & \bf{61.02}\% & 2.26\% & \bf{2.87}\% & %logs/190525_cifar100_moracle_fixed_as_2p9e4
191\% & \bf{57.98}\% & \bf{2.58}\% & \bf{4.53}\% \\ %logs/190525_cifar100_sup_moracle_fixed_as_3e4
APD($1$)&
134\% & 59.93\% & 2.12\% & 3.43\% & %logs/190513_cifar100_moracle_l1_5e4_full_tau
133\% & 56.76\% & 3.02\% & 6.20\% \\ %logs/190515_cifar100_sup_moracle_6e4
& 170\% & \bf{61.30}\% & \bf{1.57}\% & \bf{2.77}\% & %logs/190422_cifar100_moracle_2p9e4_full_tau
191\% & \bf{58.37}\% & \bf{2.64}\% & \bf{5.47}\% \\ %190515_cifar100_sup_moracle_3e4
APD($2$)&
135\% & \bf{60.74}\% & \bf{1.79}\% & 3.43\% &  %logs/190511_cifar100_moracle_reordered_base_l14e4_local_shared
130\% & 56.81\%  & \bf{2.85}\% & \bf{5.73}\% \\ %logs/190515_cifar100_sup_moracle_6e4_local_sharing
&
153\% & \bf{61.18}\% & \bf{1.86}\% & \bf{3.13}\% &  %logs/190511_cifar100_moracle_reordered_base_local_shared
182\% & \bf{58.53}\% & \bf{2.75}\% & \bf{5.67}\% \\  %logs/190516_cifar100_sup_moracle_3e4_k3n10_local_sharing
\end{tabular}
\label{tab:full_table}
\vspace{-0.2in}
\end{center}
\end{table*}

% CIFAR100-SUPER
% ORACLE: l1=3e-4 / 6e-4
% ORACLE-LS: l1=3e-4 / 5e-4   ,k=3 per 10

\input{taskorder_full}

==> full_table.tex <==
\begin{table*}
\tiny
\begin{center}
%\caption{Comparison of model.}
\caption{\small Main experiment results of all methods. The results are the mean accuracy over experiments performed on $5$ different task order sequences with $3$ random trials. STL is the single-task learing model that trains a separate network for each task independently.}
\small
\begin{tabular}{c||c|c|c|c || c|c|c|c || c|c|c|c}
\hline 
\multicolumn{1}{c||}{}&\multicolumn{4}{c||}{MNIST-Variation}&\multicolumn{4}{c||}{CIFAR100-Split}&\multicolumn{4}{c}{CIFAR100-Superclass} \\
\hline \hline
  Methods & Capacity & AUROC & AOPD & MOPD & Capacity & Accuracy & AOPD & MOPD & Capacity & Accuracy & AOPD & MOPD  \\
\hline
STL			&
1,000\% & 80.33\% & 0.85\% & 2.05\% &
1,000\% & 63.75\% & 0.98\% & 2.23\% & 
2,000\% & 61.00\% & 2.31\% & 3.33\%  \\
\hdashline
L2T &
100\%	& 71.78\% &  10.19\%	& 31.83\% & 
100\% 	& 49.29\% &  10.56\% 	& 22.23\% & 
100\% 	& 41.71\% &    8.88\% 	& 24.93\%\\
EWC &
100\%	& 73.13\% & 3.57\%	& 7.50\% & 
100\% 	& 47.23\% & 8.04\% 	& 14.57\% & 
100\% 	& 41.02\% & 7.70\% 	& 19.27\%\\
P\&C &
100\% & 73.03\% & 7.62\% & 17.35\% &
100\% & 53.54\% & 7.90\% & 16.07\% & 
100\% & 44.80\%  & 7.27\% & 17.73\%\\
RCL &
145\% & 78.66\% & 3.56\% & 8.62\% &
181\% & 54.69\% &  6.33\% & 11.40\% & 
189\% & 51.02\%  & 5.64\% & 16.00\% \\
DEN &
144\% & 80.42\% & 3.39\% & \bf{7.42}\% & 
174\% & 57.89\% & 6.11\% &10.92\% &
191\% & 51.10\% & 5.35\% & 10.33\% \\
\hline
ORACLE-Fixed	&
139\% &\bf{80.84}\% & \bf{2.31}\% & 7.78\% &
168\% & \bf{59.40}\% & \bf{2.52}\% & \bf{5.00}\% & 
126\% & \bf{54.90}\% & \bf{3.25}\% & \bf{6.40}\% \\
ORACLE&
140\% & \bf{80.76}\% & \bf{2.50}\% & \bf{6.75}\% & 
172\% & \bf{61.01}\% & \bf{2.33}\% & \bf{3.67}\% & 
125\% & \bf{56.63}\%  & \bf{2.86}\% & \bf{5.07}\% \\
\end{tabular}
\label{tab:main_table}
\vspace{-0.2in}
\end{center}
\end{table*}


==> gap_table.tex <==
\begin{table*}[ht]
\begin{center}
%\caption{Comparison of model.}
%\caption{The Order Disparity of the	task Performance(ODP)  for all datasets. We show the task order robustness(fairness) of all continual learning benchmarks by Averaged ODP and Maximum ODP.}
\caption{\small Evaluation of order-robustness of baseline models and ours. Our method achieves the highest order-robustness on all continual learning benchmark datasets by both AOPD and MOPD. For all experiments, we use five random task sequences.}
\small
\begin{tabular}{c||c|c ||c|c ||c|c}
\hline 
\multicolumn{1}{c||}{}&\multicolumn{2}{c||}{MNIST-Variation}&\multicolumn{2}{c||}{CIFAR100-Split}&\multicolumn{2}{c}{CIFAR-Superclass} \\
\hline \hline
  Methods & AOPD & MOPD & AOPD & MOPD & AOPD& MOPD\\
\hline
STL			&
%0.38\% & 0.75\% &
0.85\% & 2.05\% &
0.98\% & 2.23\% & 
2.31\% & 3.33\% \\
\hdashline
L2T &
10.19\%	& 31.83\% & 
10.56\% 	& 22.23\% & 
8.88\% 	& 24.93\%\\
EWC &
3.57\%	& 7.50\% & 
8.04\% 	& 14.57\% & 
7.70\% 	& 19.27\%\\
P\&C &
7.62\% & 17.35\% &
7.90\% & 16.07\% & 
7.27\% & 17.73\%\\
RCL &
3.56\% & 8.62\% &
6.33\% & 11.40\% & 
5.64\% & 16.00\% \\
DEN &
3.39\% & \bf{7.42}\% & 
6.11\% &10.92\% &
5.35\% & 10.33\% \\
\hline
ORACLE-Fixed	&
%\bf{1.85}\% & \bf{3.54}\% &
\bf{2.31}\% & 7.78\% &
\bf{2.52}\% & \bf{5.00}\% & 
\bf{3.25}\% & \bf{6.40}\% \\
ORACLE&
%\bf{3.20}\% & \bf{8.61}\% & 
\bf{2.50}\% & \bf{6.75}\% & 
\bf{2.33}\% & \bf{3.67}\% & 
\bf{2.86}\% & \bf{5.07}\% \\
\end{tabular}
\label{tab:gap_table}
\end{center}
\vspace{-0.1in}
\end{table*}


==> hat_barplot.tex <==
\newcommand{\howd}{7cm}
\newcommand{\hows}{-0.25in}
\begin{figure}
\begin{tabular}{c c}
%\hspace{\fows}
\includegraphics[width=\howd]{iclr_figures/191113_hat_bar.eps}&
\hspace{\hows}
\includegraphics[width=\howd]{iclr_figures/191113_apd_bar.eps}\\
\hspace{\hows}
(a) HAT &
\hspace{\hows} (b) APD(1) \\
\end{tabular}
\caption{\small Per-task accuracy for each task sequence of HAT and our model on 8 different tasks. Task sequences are randomly generated. The task of each index ($1$-$8$) is following: CIFAR10, CIFAR100, MNIST, SVHN, FashionMNIST, Traffic Sign, FaceScrub, and NotMNIST.}
\vspace{-0.15in}
\label{fig:hat_bar}
\end{figure}

==> iclr2020/iclr2020/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> main_b.tex <==
\begin{figure}
\begin{center}
\begin{tabular}{c c c c}
%\includegraphics[scale=0.7]{./figures/concept_fig.pdf}
\includegraphics[scale=0.35]{./figures/190423_concept_0.pdf} &
\hspace{-0.2in}
\includegraphics[width=2.9cm]{./figures/190423_concept2_0.pdf} &
\includegraphics[scale=0.35]{./figures/190423_concept_1.pdf} &
\hspace{-0.2in}
\includegraphics[width=2.9cm]{./figures/190423_concept2_1.pdf}\\
\multicolumn{2}{c}{(a) Order Dependent Continual Learning} &
\multicolumn{2}{c}{(b) Order Robust Adaptive Continual Learning}\\
\end{tabular}
\caption{\small \textbf{Concept:} (a) Most existing continual learning method shows significant performance disparity for each task with different task arrival sequence. However, this may be problematic when the fairness across tasks is important, especially since we cannot control the task order in a realistic setting. (b) Our model, which decomposes the model parameters into task-shared ($\bsy\sigma$) and task-adaptive parameters($\bsy\tau_t$) can learn models that is robust to the task order by constraining the effect of each update to task-generic parts of the network.}
\label{fig:concept}
\end{center}
\end{figure}

\section{Order Robust Adaptive Learning}
\subsection{Problem Setting}
We follow a common problem setting in continual learning with network expansion~\citep{PentinaA2016nips,YoonJ2018iclr,xu2018reinforced}. While notorious catastrophic forgetting can be avoided by expanding the network capacity, increasing capacity too much hinders the effect of knowledge sharing and also incurs large overhead in terms of computation and memory. Thus, an important goal for expansion-based continual learning method is to minimize the capacity increase for newly arrived tasks. 

Specifically, we denote the dataset of the $t^{th}$ task as $\calD_t = \{\bx^i_t, \by^i_t\}_{i=1}^{N_t}$, where $\bx^i_t$ is the $i^{th}$ instance, $\by^i_t$ is its associated label vector, and $N_t$ is the number of examples for task $t$. We consider deep networks with $L$ layers where $\bsy\Theta_t = \{\bsy\theta_t^l\}$ represents the set of weights $\bsy\theta_t^l \in \Real^{d_{in} \times d_{out}}$ for each layer $l$. For notational simplicity, we suppress the layer index $l$ and denote by $\bsy\theta_t$ when the context is clear. 

In order to minimize the effect of catastrophic forgetting and network capacity expansion, we propose to decompose $\bsy\theta_t$ into a \emph{task-shared} parameter and a \emph{task-adaptive} parameter, that is, $\bsy\theta_t = \bsy\sigma + \bsy\tau_t$.
This decomposition allows to easily control the trade-off between semantic drift and predictive performance of a new task by imposing separate regularizations on decomposed parameters. When a new task arrives, we encourage the shared knowledge to be properly updated, but not too much from the previous shared parameters. At the same time, we enforce the capacity of $\bsy\tau_t$
as minimal as possible. Since we do not have access to historical data, a naive update of shared parameter will induce semantic drift for previous tasks and make the arrival order indeed matter. In order to provide order-robustness, we rather impose additional regularization preventing \emph{parameter-level} drift without explicitly referring to the loss functions of previous tasks. With this additional regularization, our method is able to adjust the knowledge sharing considering the relevance between new and old tasks, which makes our model less sensitive to the task arrival order.

%\subsection{Task-Adaptive Continual Learning with Sparse Low-Rank Matrices}
\subsection{Task-Adaptive Continual Learning}
Before describing our final objective for order-robust continual learning in Section \ref{subsec:order_robustness}, we first introduce the basic learning objective with parameters decomposed into task-shared and task-adaptive parameters:
\begin{align}
\begin{split}
	\minimize_{\bsy\sigma, \bsy\tau_t} \quad
	-\frac{1}{N_t}\sum_{i=1}^{N_t} \log p  (\by_t^i \mid \bx_t^i ; \{\bsy\sigma  +\bsy\tau_t\}) 
+\lambda_1\|\bsy\tau_t\|_1 +\lambda_2\|\bsy\sigma - \bsy\sigma^{(t-1)}\|^2_2,
\label{eq:obj_decomposition}
\end{split}
\end{align}
%\label{eq:obj_lowrank}
where $\bsy\sigma^{(t-1)}$ denotes the shared parameter before arrival of the current task $t$, $\|\cdot \|_1$ indicates an element-wise $\ell_1$ norm defined on matrix input, and $\lambda_1$, $\lambda_2$ are hyperparameters balancing between efficiency vs. accuracy/order-robustness. We empirically found that we can achieve a better local optimum of \eqref{eq:obj_decomposition} by initializing task-adaptive parameter $\bsy\tau_t$ using the task-shared parameter. This initialization strategy for task-adaptive parameter is reasonable since it allows task-adaptive parameter to be updated starting from a subspace of shared-parameter, which is our best guess before actual learning. 

%$\lambda > 0$ is a hyperparameter deciding the amount of semantic drift and $m$ is the maximum rank of task-adaptive weights, which controls a degree of network expansion.
%Since directly optimizing the rank constrained objective \eqref{eq:obj_decomposition} is NP-hard, $\bsy\tau_t \in \Real^{d_{\textrm{in}} \times d_{\textrm{out}}}$  is factorized into a product of low-rank matrices: $\bP_t\bQ_t^\top$ where $\bP_t \in \Real^{d_{\textrm{in}} \times m}$ and  $\bQ_t \in \Real^{d_{\textrm{out}} \times m}$. 
Notice that to prevent drastic change of  weights that might bring catastrophic forgetting, we simply adopt a $\ell_2$ transfer regularization for the task-shared parameter which is generally used in continual learning methods. %Yet, it is possible to apply other types of regularizations as well, such as Elastic Weight Consolidation (EWC)~\cite{kirkpatrick2017overcoming}.
And, the regularization on task-adaptive parameter restricts the maximum number of 
neurons to be added in the learning process of a new task. 


%In addition to restricting the rank of task-adaptive $\bsy\tau_t$, we also impose element-wise $\ell_1$ constraints on the low-rank factors $\bP_t$ and $\bQ_t$, to select only meaningful features and further reduce the burden of storing them. Then, our optimization problem can be slightly modified as follows:

%where $\|\cdot \|_1$ indicates an element-wise $\ell_1$ norm defined on matrix input, and $\lambda_1$, $\lambda_2$ are hyperparameters balancing the relative importances of different terms. We empirically found that we can achieve a better local optimum of \eqref{eq:obj_decomposition} by initializing low-rank factors $\bP_t$ and $\bQ_t$ using the singular value decomposition of task-shared parameter. Specifically, we first perform the singular value decomposition of task-shared learned from previous time step, $\bsy\sigma^{(t-1)} = \bU\bSigma\bV^\top$, and initialize task-adaptive parameter as $\bsy P_t = \bU\bSigma^{1/2}$ and $\bsy Q_t = \bV\bSigma^{1/2}$, respectively.  
%where $\bU \in \Real^{d_{\textrm{in}} \times m}$, $\bV \in \Real^{d_{\textrm{out}} \times m}$ are composed of left and right singular vectors, and $\bSigma \in \Real^{m \times m}$ denotes a diagonal matrix with singular values.

As shown in the experimental section, the parameter decomposition itself in \eqref{eq:obj_decomposition} helps tackle task-order sensitivity mainly because semantic drift occurs only through the task-shared parameter which is likely to correspond to more \emph{generic} features, while keeping the task-adaptive representations for the previous tasks intact. In the next section, we introduce an additional measure way of achieving task-order robustness by leveraging this decomposition.

% since a capacity of \emph{AP} 
%is able to be dynamically determined for a new task,
%due to the decomposition of weights into \emph{SP} and 
%\emph{AP}. To further enhance the robustness of 
%task order, we update \emph{AP} of previous tasks
%after training \emph{SP} for a new task,
%which is introduced in the next section.

\subsection{Order-Robustness Continual Learning}
\label{subsec:order_robustness}
An additional measure to achieve order-robustness is to re-learn task adaptive parameters of the past tasks to reflect the updates in the shared parameters at each training step, so that all previous tasks are able to maintain their original performance. Since we do not have access to data for the previous tasks, we prevent the drift at the parameter level. Toward this objective, when a new task $t$ arrives, we first recover all previous parameters ($\bsy\theta_i$ for $i<t$):
%We describe how to update \emph{AP} of old tasks without explicitly keeping data of previous ones. Due to the decomposition of network parameters into \emph{SP} and \emph{AP}, it is possible to maintain the network parameter ($\bsy\theta_i$ for $i<t$):
\be
\bsy\theta_i^* & = & \bsy\sigma^{(t-1)} + \bsy\tau_i^{(t-1)}
\label{eq:ICF_concept}
\ee
where $\bsy\tau_i^{(t-1)}$ is a task-adaptive parameter of task $i$
before training current task $t$.  Then, we update all parameters including $\bsy\sigma$ and $\{\bsy\tau_i\}_{i=1}^{(t-1)}$ under some additional regularizations: $\|\bsy\theta_i^* - \bsy\sigma + \bsy\tau_i\|_2^2$.
%Now, we are able to update \emph{AP} of previous and current tasks, while keeping old information as $\|\bsy\theta_i^* - \bsy\sigma + \bsy\tau_i\|_2^2$, where $\bsy\tau_i^{\textrm{new}}$ denotes the updated \emph{AP} of old tasks.

Another important ingredient of our method is the \emph{task-specific binary masks}, $\{\mathcal{M}_i \}_{i=1}^{T}$ as gatekeepers of knowledge sharing since imposing exactly the same task-shared parameter across all tasks requires that all tasks should be closely related with each other, which might be too stringent in practice. For each task, this binary mask is maintained along with a task-adaptive parameter in our learning framework, but the additional memory overhead is negligible since it is basically a set of binary indices.  

%Moreover, we partially update shared parameter with  
%task-specific binary masks, that is $\{\mathcal{M}_i \}_{i=1}^{T}$,
%to minimize each task's effect on the shared parameter, which is inspired by the \emph{selective retraining} procedure from \cite{YoonJ2018iclr}. 
 
We apply binary masks to output channels or neurons of the task-shared parameters in each layer of the neural network: 
$\bsy\sigma \otimes \calM_i$.
For continuous relaxation to binary masks, we represent the mask as a logistic function with learnable parameters $\bv_i$  
\footnote{It is also possible to use a stochastic mask by leveraging the reparameterization trick on Bernoulli distribution~\citep{GalY2017nips}. Yet, in our formulation,
we observe that a sigmoid relaxation performs reasonably well and comparable to its stochastic counterpart.}. 
Then, the recovery procedure of previous parameters in \eqref{eq:ICF_concept} is correspondingly modified into:
\be
\bsy\theta_i^* & = & \bsy\sigma^{(t-1)}\otimes\mathcal{M}_i + \bsy\tau_i^{(t-1)}.
\label{eq:ICF_bianry_concept}
\ee
%where $\mathcal{M}_i = \textrm{sgm}(\bv_i)$ for $i < t$,
%$\bv_i$ means a trainable vector,
%and $\textrm{sgm}$ represents a logistic function. 
for tasks $i<t$. The masking functions as an \emph{attention} on the task-shared parameter to guide the learner to focus only on the parts relevant for each task, thus minimizing the drift which will help with both the prevention of catastrophic forgetting and order-robustness.

Now, we introduce our final objective function:
\begin{align}
\begin{split}
&\minimize_{\bsy\sigma, \{\bsy\tau_i\}_{i=1}^{t}, \bv_{1:t}}
\ \mathcal{L}\left(\calD_t ; \bsy\sigma\otimes\mathcal{M}_t 
+\bsy\tau_t\right) +  \lambda_1 \mathcal{S}_{1:t}
+\sum^{t-1}_{i=1}\left[\lambda_2\|\bsy\theta^{*}_i - (\bsy\sigma \otimes
\mathcal{M}_i  + \bsy\tau_i)\|^2_2 \right],
\label{eq:oracle}
\end{split}
\end{align}
%+ \lambda_3 \|\mathcal{M}_i \|_1\right],
where we use $\mathcal{L}$ to denote the standard loss function, $\mathcal{M}_i = \textrm{sgm}(\bv_i)$ using sigmoid function, and 
%$\bsy\tau_i = \bP_i\bQ_i^\top$,
%$\bsy\theta^{*}_t$ is a constant $\bsy\theta^{*}_t = \bsy\sigma^{(t-1)} \otimes\mathcal{M}_i + \bsy\tau_i^{\textrm{(t-1)}}$, 
%and  $\mathcal{M}_i = \textrm{sgm}(\bv_i)$, for all $i=1,\cdots,t$.
the sparsity-inducing penalty term $\mathcal{S}_{1:t}$ is 
defined as %below:
%\be
$\mathcal{S}_{1:t}=\sum^t_{i=1}\left(\|\bsy\tau_i\|_1\right)$.
%\label{eq:sparsity}
%\ee
This order-robust learning procedure is illustrated in Figure~\ref{fig:illustration_oracle} and is formally described in Algorithm~\ref{alg:main_alg}.



Compared to \eqref{eq:obj_decomposition}, the task-adaptive parameter of previous tasks are
not fixed during update for each task. This allows us to properly 
learn a new meaningful shared parameter and to provide the order-robustness by minimizing the mismatch between the new shared parameter and the old task-adaptive parameters. We name our final algorithm as \emph{ORACLE} (Order Robust Adaptive Continual LEarning) and its simplified version as \emph{ORACLE-Fixed}. In \emph{ORACLE-Fixed}, we only solve \eqref{eq:obj_decomposition} without any update for earlier task-adaptive parameters or applying the binary masks.  

%task-adaptive parameters for earlier tasks, which is more robust to the task
%arrival order. We refer to this formulation as ORACLE (Order Robust Adaptive Continual LEarning), and Eq.~\ref{eq:final_lowrank} as \emph{ORACLE-Fixed}, since
%for the latter the learned $\bsy\tau_i$ is fixed and without any update after training for the task $i$.


\begin{algorithm}[t]
\small
\caption{Pseudo-code of ORACLE}
\label{alg:main_alg}
\begin{algorithmic}[1]
\INPUT $\mbox{Dataset}~\calD_{1:T} ~\mbox{and hyperparameter}~\lambda, m$
\OUTPUT $\bsy\sigma^{(T)},~\mbox{and}~\bsy\tau_{1:T}$
\STATE Optimize $\bsy\theta_1$ for the task 1
\STATE Let $\bsy\sigma^{(1)} = \bsy\theta_1$
\FOR{$t=2,...,T$}
	\FOR{$i=1,...,t-1$}
		\STATE Restore $\bsy\theta_i^\ast = \bsy\sigma^{(t-1)}
							+\bsy\tau^{(t-1)}_i$ %\bP_i^{(t-1)}[\bQ_i^{(t-1)}]^\top$
	\ENDFOR	
	\STATE Initialize $\bsy\tau_t=\bsy\sigma^{(t-1)}$
	%$\bP_t = \bU\bSigma^{1/2}$ and $\bQ_t = \bV\bSigma^{1/2}$,
	%where $\bU, \bSigma, \bV = \textrm{SVD}(\bsy\sigma^{(t-1)})$
	\STATE Minimize \eqref{eq:oracle} to update $\bsy\sigma$ and $\{\bsy\tau_i, \mathcal{M}_i\}_{i=1}^{t}$
\ENDFOR

\end{algorithmic}
\end{algorithm}

\rec{\subsection{Graceful Task Forgetting}}
Since we are living in the real-world where should be suffered from finite resource issue, all of us are always required to choose much important information under our finite memory. Analogously, even continual  learning aims to lifelong knowledge training that the model can learn over and over, we might need to select a few of core information if the memory capability is over. In these respects, flexible task knowledge drop is practically important. If we learnt some tasks long time ago, and we don't need them anymore, removing the useless knowledge in our memory is necessary. Unfortunately, conventional continual learning work including both fixed-sized, and expandable, couldn't deal with this problem at all. If we force to remove the knowledge of prior tasks, inherently it must hurt information of other innocent tasks. However, our proposed model, ORACLE easily gets rid of the useless tasks without any risk. This is came from our unique architectural property: decomposition as task-shared and task-adaptive parameters. Deleting knowledge of learnt task $k$ in ORACLE is equal to delete only task-adaptive parameter $\bsy\tau_k$, and naturally, since each task-adaptive parameter is semantically and architecturally independent, the model can successfully remove it.


==> main_table.tex <==
\begin{table}[ht]
\caption{Main experiment results of all methods.}
\begin{center}
\small
%\caption{Comparison of model.}
\begin{tabular}{c|c|c|c}
\hline \hline
\multicolumn{4}{c}{MNIST-Variation} \\
\hline \hline
  Methods & Capacity & AUROC & Perf. Gap\\
\hline
  STL			& 1,000\%	& 80.48\% & 0.46\%\\
\hdashline
  L2T 		& 100\%	& 73.01\% & 4.17\%\\
  P\&C ($L_2$) & 100\%	& 73.36\% & -.--\%\\
  RCL 		& 147\%	& 77.60\% & 2.36\%\\
  DEN		& 141\% 	& 80.62\% & 4.48\%\\
\hline
  ORACLE-Fixed& 140\% & 80.55\%& 2.19\%\\
%  ORACLE 		& 139\% & 81.16\% & -.-x  & 2.30\%\\
%  M-ORACLE 	& \rec{143}\% & \rec{79.94}\% & -.-x  & \rec{1.96}\%\\
  ORACLE & \bf{139}\% & \bf{81.76}\%  & \bf{2.00}\%\\



\hline \hline
\multicolumn{4}{c}{CIFAR-100 Split} \\
\hline \hline
  Methods & Capacity & Accuracy & Perf. Gap\\
\hline
  STL			& 1,000\%	& 63.83\% &0.98\%\\
\hdashline
  L2T  & 100\% 	& 49.09\% & 6.38\%\\
  P\&C ($L_2$) & 100\%	& --.--\% & -.--\%\\
  RCL 	 		& 178\%	& 55.36\% & 4.79\%\\
%  DEN\cite{YoonJ2018iclr}& 195\% 	& 59.12\% & -.-x & 6.39\%\\
  DEN & 174\% 	& 57.97\% & 6.39\%\\
\hline
	%  F-ORACLE 	& 184\% & 59.08\% & -.-x & 1.60\%\\
  ORACLE-Fixed	& 170\% & 59.37\% & 1.92\%\\
%  ORACLE 		& 165\% & 60.02\% & -.-x & 1.59\%\\
%  ORACLE (Adaptive Masking) 	& 167\% & 58.87\% & -.-x & 1.24\%\\
  ORACLE	& \bf{168}\% & \bf{60.96}\% & \bf{1.56}\%\\



\hline \hline
\multicolumn{4}{c}{CIFAR-100 Superclass} \\
\hline \hline
  Methods & Capacity & Accuracy & Perf. Gap\\
\hline 
  STL			& 2,000\%	& 60.89\%  & 1.70\%\\
\hdashline
  L2T 		& 100\% 	& 41.77\% & 5.18\%\\
  P\&C ($L_2$) & 100\%	& --.--\% & -.--\%\\
  RCL & 194\%	& 50.71\%& 3.57\%\\
  DEN & 195\% 	& 51.16\% & 4.81\%\\

\hline
  ORACLE-Fixed & 123\% & 54.81\%  & 2.23\%\\
 % ORACLE 	& 133\% & 55.61\% & -.-x & 2.18\%\\
  %ORACLE 	& 120\% & 55.87\% & -.-x & 2.62\%\\
  ORACLE & \bf{120}\%  & \bf{56.20}\%  & \bf{1.77}\%\\
\hline \hline
\end{tabular}
\end{center}
\label{tab:m_table}
\end{table}


==> main_table3.tex <==
\begin{table*}
\begin{center}
%\caption{Comparison of model.}
\caption{\small Main experiment results of all methods. The results are the mean accuracy over experiments performed on $5$ different task order sequences with $3$ random trials. STL is the single-task learing model that trains a separate network for each task independently. \jh{Standard deviation is included in~\ref{tab:abl_table}.}}
\small
\begin{tabular}{c||c|c || c|c || c|c}
\hline 
\multicolumn{1}{c||}{}&\multicolumn{2}{c||}{MNIST-Variation}&\multicolumn{2}{c||}{CIFAR100-Split}&\multicolumn{2}{c}{CIFAR100-Superclass} \\
\hline \hline
  Methods & Capacity & AUROC & Capacity & Accuracy & Capacity & Accuracy \\
\hline
STL			&
1,000\% & 80.33$\pm$0.04\% &
1,000\% & 63.75$\pm$0.11\% & 
2,000\% & 61.00$\pm$0.09\%  \\
\hdashline
L2T &
100\%	& 71.78$\pm$0.99\% & 
100\% 	& 49.29$\pm$0.29\% & 
100\% 	& 41.71$\pm$0.30\% \\
EWC &
100\%	& 73.13$\pm$2.70\% & 
100\% 	& 47.23$\pm$3.06\% & 
100\% 	& 41.02$\pm$0.81\% \\
P\&C &
100\% & 73.03$\pm$0.61\% & 
100\% & 53.54$\pm$0.73\% &
100\% & 44.80$\pm$0.35\%  \\
RCL &
145\% & 78.66$\pm$0.37\% & 
181\% & 54.69$\pm$0.14\% & 
189\% & 51.02$\pm$0.19\%  \\
DEN &
144\% & 80.42$\pm$0.31\% & 
174\% & 57.89$\pm$0.15\% & 
191\% & 51.10$\pm$0.22\% \\
\hline
ORACLE-Fixed	&
%141\% & 80.85$\pm$0.38\% &
139\% &\bf{80.84}$\pm$\bf{0.30}\% &
168\% & 59.40$\pm$0.13\% &
126\% & 54.90$\pm$0.24\% \\
ORACLE&
%138\% & \bf{81.45}$\pm$\bf{0.17}\% &
%145\% & \bf{81.31}$\pm$\bf{0.23}\% &
140\% & 80.76$\pm$0.26\% &
172\% & \bf{61.01}$\pm$\bf{0.07}\% & 
125\% & \bf{56.63}$\pm$\bf{0.14}\%  \\
\end{tabular}
\label{tab:main_table}
%\vspace{-0.2in}
\end{center}
\end{table*}


==> mainresult2.tex <==
\begin{figure*}[ht]
\small
\begin{center}
\begin{tabular}{l c r}
%\includegraphics[width=4.7cm]{figures/190119_mnistV_perf_over_capacity.eps}&
%\includegraphics[width=4.7cm]{figures/190119_cifar100_perf_over_capacity.eps}&
%\includegraphics[width=4.7cm]{figures/190119_cifar100_sup_perf_over_capacity2.eps}\\
%\includegraphics[width=4.7cm]{figures/190119_mnistV_perf_over_time.eps}&
%\includegraphics[width=4.7cm]{figures/190119_cifar100_perf_over_time2.eps}&
%\includegraphics[width=4.7cm]{figures/190119_cifar100_sup_perf_over_time2.eps}\\
\includegraphics[width=4.3cm]{figures/190124_mnistV_robust_ver_perf_over_capacity.eps}&
\includegraphics[width=4.3cm]{figures/190122_cifar100_over_capacity.eps}&
\includegraphics[width=4.3cm]{figures/190122_cifar100_sup_over_capacity.eps}\\
\includegraphics[width=4.3cm]{figures/190124_mnistV_robust_ver_perf_over_time.eps}&
\includegraphics[width=4.3cm]{figures/190124_cifar100_perf_over_time.eps}&
\includegraphics[width=4.3cm]{figures/190124_cifar100sup_perf_over_time.eps}\\
(a)MNIST-Variation (T=10) & (b) CIFAR-100 Spl.(T=10)  & (c) CIFAR-100 Super.(T=20) \\
\end{tabular}
\end{center}
\caption{\small Accuracy over efficiency of expansion-based continual learning methods and our methods. \textbf{Top row:} Performance over capacity on all datasets. \textbf{Bottom row:} Performance over training time on all datasets.}
\label{fig:main_fig}
\end{figure*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> mv_table.tex <==
\begin{table}[ht]
\tiny
\begin{center}
%\caption{Comparison of model.}
\caption{\small Experiment results of all methods on MNIST-Variation dataset. The results are the mean AUROC over experiments performed on $5$ different task order sequences with $3$ random trials.}
\small
\begin{tabular}{c|| c|c|c|c}
\hline 
%\multicolumn{1}{c||}{}&\multicolumn{4}{c}{MNIST-Variation} \\
%\hline \hline
  Methods & Capacity & AUROC & AOPD & MOPD \\
\hline
\hline

STL			&
1,000\% & 80.33\% & 0.85\% & 2.05\% \\
\hdashline
L2T &
100\% 	& 73.87\% &  10.06\% 	& 23.30\%\\
EWC &
100\% 	& 76.69\% & 6.40\% 	& 12.43\%\\
P\&C &
100\% & 76.52\%  & 5.89\% & 11.57\%\\
PGN &
162\% & 79.47\%  & 2.70\% & 10.47\%\\
DEN &
144\% & 80.42\% & 3.39\% & 7.42\% \\
RCL &
145\% & 78.66\%  & 3.56\% & 8.62\% \\
\hline
HDN(1)	&
%139\% & \bf{80.84}\% & \bf{2.31}\% & 7.78\% \\
143\% & \bf{80.81}\% & \bf{1.61}\% & \bf{4.03}\% \\
HDN(2) &
%140\% & \bf{80.76}\%  & \bf{2.50}\% & \bf{6.75}\% \\
131\% & \bf{80.57}\%  & \bf{2.24}\% & \bf{6.01}\% \\
\end{tabular}
\label{tab:mv_table}
\vspace{-0.2in}
\end{center}
\end{table}


==> old_introduction.tex <==
\section{Introduction}
Continual learning~\citep{ThrunS1995}, or lifelong learning, is a learning scenario where a model is incrementally updated over a sequence of tasks, potentially performing knowledge transfer from earlier tasks to later ones. Building a succesful continual learning model may lead us one step further to building a general artificial intelligence, since the learning over numerous tasks in a long-term time period is an inportant aspect of human intelligence. Continual learning is often formulated as an incremental / online multi-task learning that models complex task-to-task relationships, either by sharing basis vectors in linear models~\citep{KumarA2012icml,RuvoloP2013icml} or weights in neural networks~\citep{LiZ2016eccv}. One problem that arises here is that as the model learns on the new tasks, it could forget what it learned for the earlier tasks, which is known as the problem of catastrophic forgetting. Thus an effective continual learning method should obtain a good performance using the knowledge of earlier tasks, while also retaining performances on old tasks.

Many recent work in continual learning of deep networks~\citep{LiZ2016eccv,LeeS2017nips,ShinH2017nips,kirkpatrick2017overcoming} tackle this problem by introducing advanced regularizations to prevent drastic change of network weights, while fully utilizing its capacity. Yet, when the model should adapt to new tasks that are largely different from old ones, or adapt to large number of tasks, the initial network capacity may be insufficient to accurately represent these newly observed tasks. Thus, a dominant approach nowadays is to allow the network to expand its capacity as they adapt to new tasks~\citep{RusuA2016nips,FangY2017ijcai,YoonJ2018iclr}. These recent advances in continual learning have largely alleviated the catastrophic forgetting problem, \rec{but still the issue remains.} %to the point that it is no longer a serious problem. 

\begin{figure}
\begin{center}
\begin{tabular}{c c c c}
%\includegraphics[scale=0.7]{./figures/concept_fig.pdf}
\includegraphics[scale=0.35]{./figures/190423_concept_0.pdf} &
\hspace{-0.2in}
\includegraphics[width=2.9cm]{./figures/190423_concept2_0.pdf} &
\includegraphics[scale=0.35]{./figures/190423_concept_1.pdf} &
\hspace{-0.2in}
\includegraphics[width=2.9cm]{./figures/190423_concept2_1.pdf}\\
\multicolumn{2}{c}{(a) Order Dependent Continual Learning} &
\multicolumn{2}{c}{(b) Order Robust Adaptive Continual Learning}\\
\end{tabular}
\caption{\small \textbf{Concept:} (a) Most existing continual learning method shows significant performance disparity for each task with different task arrival sequence. However, this may be problematic when the fairness across tasks is important, especially since we cannot control the task order in a realistic setting. (b) Our model, which decomposes the model parameters into task-shared ($\bsy\sigma$) and task-adaptive parameters($\bsy\tau_t$) can learn models that is robust to the task order by constraining the effect of each update to task-generic parts of the network.}
\label{fig:concept}
\end{center}
\end{figure}

Simultaneously, there is one another important problem that has been relatively neglected in previous work on continual learning, which we name as the \emph{task order dependency} problem, which describes the issue that the order of task arrival sequence has large impact on the performance of individual task as well as on the overall performance. The bar plots in Figure~\ref{fig:concept}(a) illustrates this situation.  Such high sensitivity of task-specific performance according to the task arrival sequence could be highly problematic if fairness across tasks is important (e.g. disease diagnosis). Curriculum learning is one way to resolve this task order dependency problem; however, in most real-world scenarios it is often not possible to control the order the model learns on new tasks. For example, a product identification system should train to recognize new products in a timely manner without knowing what products will arrive at the market next. \rec{Naturally, This problem gets much vicious as many tasks arriving.}

\rec{Thus, to resolve both issues; catastrophic forgetting and ensure fairness among tasks at once, a continual learning model should be order-robust.} But how can we obtain a model that is inherently robust to the order of the task sequence, without knowing what tasks will arrive in the future? The main reason existing continual learning methods obtain task order-sensitive models, is because the change in the model parameters affect all previous tasks, as the model drifts away from the initial solution (See Figure~\ref{fig:concept}(a)). To prevent this, we propose a model that decomposes the parameters into task-shared and task-specific parameters. With this decomposition, the task-shared parameters, which contain features of generic importance could stay relatively static with the arrival of new tasks, since the new tasks will mostly learn the task-adaptive parameters to explain the incremental difference that cannot be explained with the task-shared parameters (Figure~\ref{fig:concept}(b)). Yet, since the task-shared parameters should also be updated to reflect the new knowledge obtained on new tasks, we allow to update the task-adaptive parameters for old tasks to reflect the changes in the task-shared parameters. Our model, Order-Robust Adaptive Continual LEarning (ORACLE), obtains similar performance for all tasks regardless of the order of the task sequence (Figure~\ref{fig:concept}(b)).  

ORACLE, unlike existing continual learning methods with network expansion, can expand the capacity of the network with simple matrix computation when necessary without having to go over complex re-training steps or training of agents using reinforcement learning, and thus is considerably more lightweight in terms of computation. \rec{As a result, only ORACLE practically carries out even the \emph{extreme continual learning} scenarios which the model takes more than 100 tasks, among expandable continual learning algorithms.}

\rec{Nevertheless our objective is to build lifelong trainable continual learning model, this can be considered too ideal since the capability is inevitably finite in the real-world. This is also an identical limitation on both non-mammalian and mammalian brain. To prevent the exploding information over their capability, they effectively remove less important knowledge. Absolutely, we know that \emph{human is an expert of the Forgetting}. How about the continual learning algorithms? Unfortunately, most of conventional work might not consider this fundamental subject. Basically, they have no explicit distinction of features among tasks, in other words, there is no way to remove specific task information from mixed up knowledge pool without disturbing other tasks'. On the other hand, our ORACLE can perform graceful task forgetting as a duck takes to water. The ability is from its unique architectural characteristics; parameter decomposition. Since each task-adaptive parameters are semantically independent, even if several tasks' knowledge is dropped, there is no undesired forgetting of innocent tasks.}

We validate our methods on several benchmark datasets for continual learning while comparing against state-of-the-art continual learning methods with or without network expansion, and obtain significantly superior performance to them with minimal increase in network capacity and only a fraction of computations required for previous network expansion methods. Further validation of our method on order-robustness shows that our model is significantly more robust to the order of the task arrival sequence compared to existing methods as well. Besides, we show meaningful validations about graceful task forgetting, and extreme continual learning scenarios.

%"REMINDING"
%Naturally, if the learner absorbed the features of several independent tasks at different times, there shouldn't be any hierarchy among the information. In other words, optimal continual learning scenarios, the learned information of different tasks can be complementary but not be dependent. However, we observe that the task-order on the continual learning can be a truly sensitive hyperparameter and most of current research also suffers from this problem. We define the issue as \emph{Task-order Dependency} on continual learning, and present the novel approach to mitigate this problem in our work. At the core, we formulate the algorithm as two stage. At the first stage, the model trains current task without any transfer constraints which is one of the main reason of the \emph{task-order dependency}. At the second stage, all of the learned \emph{SP} and \emph{AP} are refined to prevent the catastrophic forgetting and find the optimal volume of the expanded capacity.



The contribution of this paper is threefold:

\begin{itemize}
	\item We tackle a novel and a critical issue in continual learning, \emph{task-order dependency}, which describes the situation where the task performance changes sensitively to the order of the task arrival sequence, and propose metrics to measure order-sensitivity in continual learning.

	\item We introduce a simple and generic framework for continual deep learning that can effectively tackle the problem of task-order dependency, that is also highly efficient in terms of memory and computation.
	
	\item \rec{We suggest another novel continual learning issues named \emph{graceful task forgetting}, and \emph{extreme continual learning}, and the proposed model outstandingly solve both problem unlike other benchmarks.}
	
	%\item We conduct extensive continual learning experiments to validate that the proposed network outperforms existing expandable networks with considerably fewer number of parameters and significantly less training time, as well as obtains results that is order-robust, to further ensure fairness among tasks.  
\end{itemize}


==> old_related_work.tex <==
\section{Related work}

\paragraph{Lifelong / Continual Learning}
The literature on continual (lifelong) learning~\citep{ThrunS1995} is vast~\citep{RuvoloP2013icml} as it is a long-studied topic; however, due to space limitation we only mention recent deep learning-based methods. In the past, the subject of interest for continual learning was how to transfer knowledge from earlier task to later ones. Yet, this is less of a challenge with (deep) neural networks, since a new task can easily access the knowledge from the old tasks via the learned network weights. Thus, instead of knowledge transfer, most continual deep learning approaches are focused on preventing \emph{catastrophic forgetting}, in which case the retraining of the network for new tasks shifts the distribution of the learned representation, and degenerates the performance on the earlier tasks. A common practice to alleviate catastrophic forgetting is to introduce regularizers that prevent significant changes of model parameters when learning for a new task. A simple yet effective regularization is to enforce the representations learned at the current task to be closer to one from a previous task network as much as possible~\citep{LiZ2016eccv}. A more advanced approach is to employ deep generative models that encode previous task knowledge in a compact description~\citep{ShinH2017nips}, to be used later when learning for a novel task. \cite{kirkpatrick2017overcoming} proposed to regularize the model parameter for the current tasks with parameter for the previous task via Fisher information matrix, to find a solution that works well for both tasks, and \cite{LeeS2017nips} introduces a moment-matching technique with a similar objective. \cite{CuongN2018iclr} formulates continual learning as a sequential Bayesian update, which introduces a coreset (i.e. a small subset of datasets) of each observed task to summarize the old information to mitigate forgetting, when estimating the posterior distribution over weights given the current task. P\&C~\citep{schwarz2018progress} splits a complex continual learning step into progress and compression phases. In the progress stage, a small network referred to as the adaptor is introduced to solve the new task, and in the compression phase, the newly learned information is merged into the main network through the knowledge distillation~\citep{HintonG2014nipsw} while preventing semantic drift. 


% \cite{PentinaA2016nips} aggregates base classifiers learned from previous tasks with weighted majority voting to leverage knowledge transfer, providing a full analysis of generalization performance on the voting-based algorithm, but it is not clear how to keep previous hypotheses in a compact form, which limits practical usability.

\iffalse
\begin{table}[t]
\small
\center
\caption{Comparison of the proposed method against existing continual learning methods with respect to catastrophic forgetting, network expandability, and order fairness.}
\vspace{.05in}
\begin{tabular}{c|c|c|c}
\hline \hline
  Methods & Forgetting & Expandable  & Order Fairness\\
\hline
  PRN & N & Y & N\\
  P\&C & Y (Minimal) & N & N \\
  RCL & N & Y (Dynamic) & N \\
  DEN & Y(Minimal) & Y (Dynamic) & N\\
\hline
  ORACLE & Y (Minimal) & Y (Dynamic) & Y\\
\hline \hline
\end{tabular}
\label{tab:comp}
\end{table}
\fi

\iffalse
\begin{table*}[ht]
\small
\center
\caption{Comparison of the proposed network with relevant methods with respect to accessibility of previous task information, semantic drift, network expandability, and order fairness.}
\vspace{.05in}
\begin{tabular}{c|c|c|c|c}
\hline \hline
  Methods & Data on Previous Tasks & Catastrophic Forgetting & Expandable  & Order Fairness\\
\hline
  IMM~\cite{LeeS2017nips} & N & Y  & N & N\\
  DGR~\cite{ShinH2017nips} & N & Y & N & N\\
  VCL~\cite{CuongN2018iclr} & Y (Coreset) & Y & N & N\\
\hline
  DMT~\cite{FangY2017ijcai} & N & N & Y & N\\
  PRN~\cite{RusuA2016nips} & N & N & Y & N\\
  P\&C~\cite{schwarz2018progress} & N & Y & N & N \\
  RCL~\cite{xu2018reinforced} & N & N & Y (Dynamic) & N \\
  DEN~\cite{YoonJ2018iclr} & N & Y & Y (Dynamic) & N\\
\hline
  Proposed Network & N & Y (Minimal) & Y (Dynamic) & Y\\
\hline \hline
\end{tabular}
\label{tab:comp}
\end{table*}
\fi


\paragraph{Dynamic Network Expansion} 
Even with such well-defined regularizers, it is nearly impossible to completely avoid catastrophic forgetting, since in practice, the model may encounter unlimited number of tasks. An effective way to tackle this challenge is by dynamically expanding the network capacity to deal with new tasks. Dynamic network expansion approaches have been introduced in earlier work such as~\cite{ZhouG2012aistats}, which proposed an iterative algorithm to train a denoising autoencoder while adding in new neurons one by one and merging similar units. In light of continual learning, \cite{RusuA2016nips} proposed to expand the network by augmenting each layer of a network by a fixed number of neurons for each task, while keeping the old weights fixed to avoid catastrophic forgetting. Yet, this approach often results in a network with excessive size, and requires manual tuning of the number of neurons to add to each layer. \cite{YoonJ2018iclr} proposed Dynamically Expandable Networks that overcome these limitations via selective retraining of the old network while expanding each of its layer with only the necessary number of neurons, by applying group sparsity on the incoming weights to each unit, and further alleviate catastropihc forgetting by splitting and duplicating the neurons affected by the training on the new task. \cite{xu2018reinforced} proposed to solve the network expansion problem using reinforcement learning, to find the network architecture that is compact yet performs well. Our model also perform dynamic network expansion as the previous expansion-based methods, but instead of adding in new units, it adds task-specific parameter to each unit. Further, the capacity increase is kept minimal by penalizing the sparsity inducing regularization to the task-specific parameters.

Owing to these recent advances in continual learning, catastophic forgetting is relatively less of an issue now, and thus in this work we focus more on the new problem of \emph{task order-robustness}, which to our knowledge, has not been tackled in existing work on continual learning.


==> omn_result.tex <==
\begin{figure}
\noindent\begin{minipage}{.55\textwidth}
\begin{small}
\begin{tabular}{c||c|c ||c|c}
\hline 
Models & Capacity & Accuracy & AOPD & MOPD \\
\hline
\hline
STL & 10,000\% & 82.13\%& 2.79\% & 5.70\%\\
%MTL & 2,132\% & 53.53\%& - & -\\
\hdashline

L2T & 2,132\% & 66.34\%& 11.50\% & 26.57\% \\
& 100\% & 63.46\%& 13.35\% & 24.43\% \\
%EWC & 100\% & 62.58\%& 10.98\% & 22.63\% \\
%		& 2,132\% & 62.33\%& 10.28\% & 27.83\% \\
EWC & 2,132\% & 72.06\%& 11.84\% & 31.93\% \\
& 100\% & 67.48\%& 14.92\% & 32.93\% \\
PGN  & 1,543\% & 79.35\% & 4.52\% & 10.37\%\\
%& 902\% & 73.13\% & 6.39\% & 21.10\%\\
& 1,045\% & 73.65\% & 6.79\% & 19.27\%\\
%RCL & - & - & - & -\\
%EXID & \rec{1,020}\% & \rec{79.27}\% & xx\% & xx\%\\
DN & 2,119\% & \textbf{81.21}\%& \textbf{3.44}\%& \textbf{8.05}\%\\
& 1,072\% & \textbf{79.62}\%& 4.51\%& 12.36\%\\
%logs/190428_omn_moracle_trial_sel_app_simp
%EXID-LS & \rec{992}\% & \rec{\textbf{79.67}}\%& \textbf{4.46}\%& \textbf{9.03}\%\\
HDN & \textbf{943}\% & \textbf{81.60}\%& \textbf{3.78}\%& \textbf{8.19}\%\\
& \textbf{649}\% & \textbf{81.20}\%& \textbf{4.09}\%& \textbf{9.44}\%\\
%logs/190516_omn_moracle_retry_l1_4e4_approx1K_LS_SAS
\end{tabular}
\end{small}
%\captionof{table}{Performance comparison with several benchmarks on Omniglot-rotation.}
%\label{tab:omn_table}
\end{minipage}
\hspace{0.1in}
\begin{minipage}{.4\textwidth}
%\begin{center}
%\includegraphics[height=4cm]{figures/190517_omniglot_capacity.eps} 
\includegraphics[height=4cm]{figures/190523_omniglot_capacity_increase.eps} 
%\captionof{figure}{Capacity increase during continual learning on Omniglot-rotation.}
%\label{fig:omn_plot}
\end{minipage}
\caption{\small \textbf{Left:} Performance comparison with several benchmarks on Omniglot-rotation, where the performance of DEN and RCL 
are not reported due to their inefficiencies
to large-scale continual learning. \textbf{Right:} The number of the parameters which is obtained during course of training on Omniglot-rotation.}
\label{fig:omn_results}
\vspace{-0.2in}
\end{figure}


==> param_anal_result.tex <==
\begin{figure}
\small
\begin{center}
%\hspace{-0.2in}
\begin{tabular}{c c}

\includegraphics[width=5cm]{figures/190123_foracle_l2t_norm_distance.eps}&
\includegraphics[width=5cm]{figures/190123_oracle_l2t_norm_distance.eps}\\

(a) Fixed previous $\bsy\tau$ & (b) HDN(1) \\\\
\end{tabular}
\vspace{-0.1in}
\caption{\small Amount of update in task-shared parameters as HDN(1) with fixed previous $\bsy\tau$ depicted in \textbf{A.3} and HDN(1) train on a sequence of tasks.}
\vspace{-0.2in}
\label{fig:param_anal}
\end{center}
\end{figure}

==> runtime_table2.tex <==
\begin{table}[ht]
\begin{center}
\caption{Runtime (in seconds) comparison for all methods on MNIST-Variation, CIFAR100-Split, and CIFAR100-Superclass.}
\begin{tabular}{cccc}
\hline \hline
  Methods& MNIST-Variation.  & CIFAR100-Split & CIFAR100-Super.\\

\hline
\hline
%\vspace{-0.05in}
L2T & 129 & 113 & 106\\
%\vspace{0.1in}
%\vspace{0.1in}
DEN &2590 &1624 & 2592\\
%\vspace{0.1in}
%\vspace{0.1in}
RCL &5687&2723&3381\\
\hline
ORACLE-Fixed&193&143&138\\
ORACLE&427&297&442\\
%\vspace{0.1in}
\hline \hline
\end{tabular}
\label{tab:t_table}
\end{center}
\end{table}

\iffalse
\begin{table*}[ht]
\caption{Runtime (in seconds) comparison for all methods.}
\begin{center}
\begin{tabular}{ccccccc}
\hline \hline
%\vspace{0.1in}
  Methods& L2T& P\&C & DEN & RCL & ORACLE-Fixed & ORACLE\\
%\vspace{-0.5in}
\hline
\hline
%\vspace{-0.05in}
MNIST Variation & 129 & 0 & 2590 & 5687 & 193 & 427  \\
%\vspace{0.1in}
\hline
%\vspace{0.1in}
CIFAR100 Split & 113 & 0 & 1624 & 2723 & 143 & 297  \\
%\vspace{0.1in}
\hline
%\vspace{0.1in}
CIFAR100 Superclass & 106 & 0 & 2592 & 3381 & 138 & 442  \\
%\vspace{0.1in}
\hline \hline
\end{tabular}
\label{tab:t_table}
\end{table*}
\fi


==> runtime_table3.tex <==
\begin{table}[ht]
\begin{center}
\small
\caption{Training time (in seconds)comparison for expandable continual learning methods on MNIST-Variation, CIFAR-100 Split, and CIFAR-100 Superclass, where the running time is measured on Titan X (Pascal).}
\begin{tabular}{cccc}
\hline \hline
  Methods& MNIST-Variation.  & CIFAR-100 Split & CIFAR-100 Superclass\\

\hline
\hline
%\vspace{-0.05in}
L2T & 129 & 113 & 106\\
PGN & 135 & 132 & 293\\
%\vspace{0.1in}
%\vspace{0.1in}
DEN &2590 &1624 & 2592\\
%\vspace{0.1in}
%\vspace{0.1in}
RCL &5687&2723&3381\\
\hline
%DN-Fixed&193&143&138\\
%DN&427&297&442\\
APD(1) & 242&227&382\\
APD(2) &250&235&382\\
%\vspace{0.1in}
\hline \hline
\end{tabular}
\label{tab:t_table}
\end{center}
\end{table}

\iffalse
\begin{table*}[ht]
\caption{Runtime (in seconds) comparison for all methods.}
\begin{center}
\begin{tabular}{ccccccc}
\hline \hline
%\vspace{0.1in}
  Methods& L2T& P\&C & DEN & RCL & DN-Fixed & DN\\
%\vspace{-0.5in}
\hline
\hline
%\vspace{-0.05in}
MNIST Variation & 129 & 0 & 2590 & 5687 & 193 & 427  \\
%\vspace{0.1in}
\hline
%\vspace{0.1in}
CIFAR100 Split & 113 & 0 & 1624 & 2723 & 143 & 297  \\
%\vspace{0.1in}
\hline
%\vspace{0.1in}
CIFAR100 Superclass & 106 & 0 & 2592 & 3381 & 138 & 442  \\
%\vspace{0.1in}
\hline \hline
\end{tabular}
\label{tab:t_table}
\end{table*}
\fi

